How Can Large Language Models Help Humans in Design and Manufacturing?

The advancement of Large Language Models (LLMs), including GPT-4, provides exciting new opportunities for generative design. We investigate the application of this tool across the entire design and manufacturing workflow. Specifically, we scrutinize the utility of LLMs in tasks such as: converting a text-based prompt into a design specification, transforming a design into manufacturing instructions, producing a design space and design variations, computing the performance of a design, and searching for designs predicated on performance. Through a series of examples, we highlight both the benefits and the limitations of the current LLMs. By exposing these limitations, we aspire to catalyze the continued improvement and progression of these models.

==> sections/AuxiliaryTools.tex <==
\section{Auxiliary Tools}


This is a section for describing how to enforce:

\paragraph{Visualization Tools}
Describe standard tools for:
SVG (e.g., inkscape, Gimp, Adobe Illustrator)
STL: Meshlab, or any CAD sofware
gcode: repetier, cura, IceSL
CAD formats: OpenJscad, Autodesk Fusion 360
Knitting: KnitOut?
Graph visualization tool - e.g., graph converter tool from Allan, Graphviz, Networkx

\paragraph{Output Verification Correctness Checking}

We want to make sure that the output is correct.
We need to have virtual tools to make sure that the output is valid and correct.

Tools to make sure that the output is valid:

Tools that ensure that the output is correct, can be done by human visual inspection. They can be also done by an automated tools that runs the visualizer or simulator. Show an example of such a tool and simulator.

\paragraph{Post-process Fixing Tools}

Results might not be correct. Describe tools to post-process the output. For example, making sure that things are connected. Non-overlapping. Write a simple post-processing script that fixes the incorrect results.


\paragraph{Using Solvers in an Interactive Loop}
Generate design (geometry) and boundary conditions, materials
We run FEA solver, (we report what max stress is)
LLM can draw additional conclusions from these results.


Constraint solvers (CSP) - TODO
Logical solvers - Coq
Numerical Solvers - Optimizers such as SNOPT, NLOpt, or linear algebra packages like Eigen.

\paragraph{Program Synthesizers}
Sketch, etc.

\paragraph{Simulators}
Static simulators - SimScale, tools built into CAD software
Dynamic simulators - Chrono, Mujoco, Bullet, etc.

\paragraph{Surrogate/learned models}
CLEVERER and intuitive physics types models
etc.


==> sections/GraphArrows/PerformanceAndDesignSpaceToDesign.tex <==
\section{Performance-and-Design-Space To Design (Liang and Andy)}

While generative algorithms can produce candidates for designs, there is no guarantee concerning their quality.  Computational design or inverse design is focused on producing designs that are, by some metric, as close to optimal as possible, given the constraints.  
Put in the vocabulary of the preceding sections, given a design space and performance metrics (which can define values to be optimized or constraints to be satisfied), which design in that space satisfies the given constraints and provides optimal performance?

A design generated by an LLM must therefore satisfy several constraints: \textit{1)} it must be valid,  \textit{2)}, \textit{3)} it must be performant, it must satisfy design constraints, and, in the context of manufacturing \textit{4)} it must be buildable.  With \textit{3) and 4)}, we note the persistent reality of the sim-to-real gap --- objective and constraint values may differ \textit{in silico} and \textit{in situ}.  Basic challenges involve specifications of the inverse problem to an LLM (much of which was described in previous sections), as well as generation of an efficacious algorithm for design optimization.

While LLMs cannot natively search for optimal solutions to a novel problem, they can make educated starting guesses and formulate code to be executed by function calling.  Much of this section is thus focused on prompting LLMs to generate meaningful code for problems dependent on aspects such as their parameterization support (\textit{e.g.} continuous versus discrete domains), performance objective landscape, or fabrication constraints.  

Real-world problems introduce nuanced challenges, including exploring over multiple competing objectives, difficult-to-specify objectives (such as aesthetics and objectives that depend on long-term use), and an evolving landscape of emerging methods that an LLM may not know about.  In this context, we could consider whether LLMs can propose novel strategies that free  designers from some of the typical burdens associated with the optimization pipeline.

With these considerations, we aim to investigate the following questions:

\textbf{Q1} Can GPT identify optimal designs when a design space and performance metric are provided?

 \textbf{1.1} When can GPT solve a problem analytically, and when does it need to resort to using an outside tool? (\textit{i.e.} a programmed algorithm). 
% table example 
 
 \textbf{1.2} Can GPT choose reasonable algorithms for different types of supports for constraints, objectives, and decision spaces (\textit{e.g.} continuous, discrete, binary, \textit{etc.}
% 3D printing example
% Robotics example


\textbf{Q2} Can this tool support optimization in contexts that require additional knowledge?

\textbf{2.1} Can GPT assist designers in navigating the landscape of possible trade-offs when multiple conflicting objectives are present?




\textbf{2.2} Can GPT support design exploration and optimization when the design 
space is not properly defined or fully bounded?

\textbf{2.3} Can GPT support design optimization when objectives are not easily quantifiable?

\subsection{GPT: Analytical vs. Outside Tools (Q1.1)}
We know that GPT has the ability to reason about many mathematical operations, including both algebra and calculus, which is sufficient to solve many real-world engineering problems.  We say reasoning, here, because it is not obvious that GPT is truly performing the operations; and, as we'll see, this often does yield mathematical errors.  Still, it is reasonable to wonder if its own internal reasoning is sufficient (perhaps, when augmented by search or a plugin), and when it one must resort to code and external libraries.  Each of these approaches has its own pitfalls that suggest caution for developers.

Consider the following example of maximizing the stability of a table.  For those unfamiliar, an object is statically stable when its center of mass lies within its support polygon.  One considers stability of an object to be maximized when it is still stable under as large of a perturbation as possible.  In principle, that typically means two things: 1) moving the center of mass as far away from the boundary of the support polygon as possible, 2) decreasing the experienced motion (typically caused by gravitational torquing) when perturbed.  

In the following example, the Wolfram plugin is enabled, which GPT can selectively call.

TODO: fix this math

% \begin{enumerate}
%     \item User:
%     \begin{lstlisting}
%     Let's say I want to design a table with four legs and a top.  Assume that the four legs are radially symmetric, and the top is a cylinder and the legs are cylinders.  Can you give me the equation for the center of mass of the table in x, y, and z, as a function of the natural parameters of the primitives?
%     \end{lstlisting}
%     \item GPT:
%     \begin{lstlisting}
%         Sure, let's denote the following parameters:

% �
% R is the radius of the table top.
% �
% r is the radius of each leg.
% �
% H is the height of the table top.
% ℎ
% h is the height of each leg.
% �
% ρ is the uniform density of the material the table is made of.
% The mass of the table top 
% �
% �
% �
% �
% M 
% top
% ​
%   and each leg 
% �
% �
% �
% �
% M 
% leg
% ​
%   can be calculated using the volume of a cylinder 
% �
% =
% �
% �
% 2
% ℎ
% V=πr 
% 2
%  h and the definition of density 
% �
% =
% �
% �
% ρ= 
% V
% M
% ​
%  , which gives us:

% �
% �
% �
% �
% =
% �
% �
% �
% 2
% �
% M 
% top
% ​
%  =ρπR 
% 2
%  H
% �
% �
% �
% �
% =
% �
% �
% �
% 2
% ℎ
% M 
% leg
% ​
%  =ρπr 
% 2
%  h
% The total mass of the table 
% �
% M is the mass of the top plus the mass of four legs:

% �
% =
% �
% �
% �
% �
% +
% 4
% �
% �
% �
% �
% M=M 
% top
% ​
%  +4M 
% leg
% ​
 
% The center of mass of the table in the z-direction 
% �
% �
% �
% z 
% cm
% ​
%   can be calculated by taking the weighted average of the centers of mass of the top and the legs. The center of mass of a cylinder is at its midpoint, so for the top it's at 
% �
% 2
% 2
% H
% ​
%   and for the legs it's at 
% ℎ
% 2
% 2
% h
% ​
%  . This gives us:

% �
% �
% �
% =
% 1
% �
% (
% �
% �
% �
% �
% �
% 2
% +
% 4
% �
% �
% �
% �
% ℎ
% 2
% )
% z 
% cm
% ​
%  = 
% M
% 1
% ​
%  (M 
% top
% ​
  
% 2
% H
% ​
%  +4M 
% leg
% ​
  
% 2
% h
% ​
%  )
% Since the table is radially symmetric, the center of mass in the x and y directions will be at the origin (0,0):

% �
% �
% �
% =
% �
% �
% �
% =
% 0
% x 
% cm
% ​
%  =y 
% cm
% ​
%  =0
% So the center of mass of the table is at (0, 0, 
% �
% �
% �
% z 
% cm
% ​
%  ).
%     \end{lstlisting}
% \item: User:
% \begin{lstlisting}
%     Ok.  Let's say the bounds for the height of the legs are between 1cm and 3 cm, and the height of the table is between 1 and 5 cm.  Show me an equation that would measure static stability, and find the minimum of that equation.
% \end{lstlisting}
% \item: GPT:
% \begin{lstlisting}
%     The static stability of a table can be quantified by the height of the center of mass. The lower the center of mass, the more stable the table is. Therefore, we can use the equation for 
% �
% �
% �
% z 
% cm
% ​
%   as our measure of static stability.

% To find the minimum of this equation, we can treat it as an optimization problem. We want to minimize 
% �
% �
% �
% z 
% cm
% ​
%   subject to the constraints 
% 1
% ≤
% ℎ
% ≤
% 3
% 1≤h≤3 and 
% 1
% ≤
% �
% ≤
% 5
% 1≤H≤5.

% The equation for 
% �
% �
% �
% z 
% cm
% ​
%   is:

% �
% �
% �
% =
% 1
% �
% (
% �
% �
% �
% �
% �
% 2
% +
% 4
% �
% �
% �
% �
% ℎ
% 2
% )
% z 
% cm
% ​
%  = 
% M
% 1
% ​
%  (M 
% top
% ​
  
% 2
% H
% ​
%  +4M 
% leg
% ​
  
% 2
% h
% ​
%  )
% Substituting the expressions for 
% �
% �
% �
% �
% M 
% top
% ​
%   and 
% �
% �
% �
% �
% M 
% leg
% ​
%   we get:

% �
% �
% �
% =
% 1
% �
% �
% �
% 2
% �
% +
% 4
% �
% �
% �
% 2
% ℎ
% (
% �
% �
% �
% 2
% �
% �
% 2
% +
% 4
% �
% �
% �
% 2
% ℎ
% ℎ
% 2
% )
% z 
% cm
% ​
%  = 
% ρπR 
% 2
%  H+4ρπr 
% 2
%  h
% 1
% ​
%  (ρπR 
% 2
%  H 
% 2
% H
% ​
%  +4ρπr 
% 2
%  h 
% 2
% h
% ​
%  )
% Simplifying, we get:

% �
% �
% �
% =
% �
% 2
% �
% 2
% +
% 2
% �
% 2
% ℎ
% 2
% �
% 2
% �
% +
% 4
% �
% 2
% ℎ
% z 
% cm
% ​
%  = 
% R 
% 2
%  H+4r 
% 2
%  h
% R 
% 2
%  H 
% 2
%  +2r 
% 2
%  h 
% 2
 
% ​
 
% Since 
% �
% R, 
% �
% r, and 
% �
% ρ are constants, we can treat this as a function of 
% ℎ
% h and 
% �
% H only:

% �
% (
% ℎ
% ,
% �
% )
% =
% �
% 2
% �
% 2
% +
% 2
% �
% 2
% ℎ
% 2
% �
% 2
% �
% +
% 4
% �
% 2
% ℎ
% f(h,H)= 
% R 
% 2
%  H+4r 
% 2
%  h
% R 
% 2
%  H 
% 2
%  +2r 
% 2
%  h 
% 2
 
% ​
 
% We can find the minimum of this function within the given bounds using calculus or numerical optimization methods. However, because this is a complex optimization problem, it would be best to use a numerical method.

% Let's use the Wolfram Language to find the minimum of this function within the given bounds.

% Used Wolfram
% I apologize for the inconvenience. It seems that the computation took longer than expected. This is a complex optimization problem that might require a significant amount of computational resources. Let's try a different approach.

% We can make a reasonable assumption that the minimum of the function will occur at the boundary of the constraints. This is often the case for physical systems. Therefore, we can evaluate the function at the four corners of the parameter space:

% �
% (
% 1
% ,
% 1
% )
% f(1,1)
% �
% (
% 1
% ,
% 5
% )
% f(1,5)
% �
% (
% 3
% ,
% 1
% )
% f(3,1)
% �
% (
% 3
% ,
% 5
% )
% f(3,5)
% Let's calculate these four values.

% Used Wolfram
% The four values of the function at the corners of the parameter space are:

% �
% (
% 1
% ,
% 1
% )
% =
% 2
% �
% 2
% +
% �
% 2
% 4
% �
% 2
% +
% �
% 2
% f(1,1)= 
% 4r 
% 2
%  +R 
% 2
 
% 2r 
% 2
%  +R 
% 2
 
% ​
 
% �
% (
% 1
% ,
% 5
% )
% =
% 2
% �
% 2
% +
% 25
% �
% 2
% 4
% �
% 2
% +
% 5
% �
% 2
% f(1,5)= 
% 4r 
% 2
%  +5R 
% 2
 
% 2r 
% 2
%  +25R 
% 2
 
% ​
 
% �
% (
% 3
% ,
% 1
% )
% =
% 18
% �
% 2
% +
% �
% 2
% 12
% �
% 2
% +
% �
% 2
% f(3,1)= 
% 12r 
% 2
%  +R 
% 2
 
% 18r 
% 2
%  +R 
% 2
 
% ​
 
% �
% (
% 3
% ,
% 5
% )
% =
% 18
% �
% 2
% +
% 25
% �
% 2
% 12
% �
% 2
% +
% 5
% �
% 2
% f(3,5)= 
% 12r 
% 2
%  +5R 
% 2
 
% 18r 
% 2
%  +25R 
% 2
 
% ​
 
% The minimum of these four values will give us an approximation of the minimum of the function within the given bounds. However, please note that this is an approximation based on the assumption that the minimum occurs at the boundary, which might not be the case. For a more accurate result, a more sophisticated numerical optimization method would be needed.
% \end{lstlisting}
% \end{enumerate}

While the Wolfram plugin was a natural choice for solving what appears to be a more simple analytical optimization problem, not enough time was alotted for it to complete the calculation.  (TODO: can we finish it ourselves on the website?)  Although it might seem like it would be trivial to provide Wolfram more time to complete the computation, in practice, the user has no feedback on how long the computation would take.  It is unreasonable to ask a user to wait for long periods of time without feedback, and it is unlikely that all computations would be able to provide meaningful feedback about progress.

GPT reasons that the optimum value will occur near the boundary of the constraints.  While this is correct, it does not prove its claim.  However, with this reasoning in tow, it then successfully uses the Wolfram Plugin to correctly compute the equations for the extremal values, which depend on $r$ and $R$.  Despite this, it fails to realize that certain solutions dominate others, and does not prune out bad candidates.

In follow-up, GPT is asked to perform the same optimization task but using code, choosing a reasonable, easily accessible (though not state-of-the-art) solver for the continuous valued problem) --- namely, L-BFGS-B, a second-order gradient-based optimizer.  It does not realize, however, that it can expedite the computation by providing explicit gradient computations, until prompted.  This is an issue for performance, because not all users will be intimately familiar with all optimization libraries, and they may not realize that by providing explicit gradients, the computation can be expedited.  GPT also does not elect to make use of Wolfram or Autodifferentiation for the gradient calculation, which could, in practice, lead to errors.

% \begin{enumerate}
%     \item User:
%     \begin{lstlisting}
%         Since Wolfram is having trouble, can you instead provide me code to find the optimum in the general case?
%     \end{lstlisting}
%     \item GPT:
%     \begin{lstlisting}
%         Sure, I can provide you with a Python code snippet that uses the scipy.optimize library to find the minimum of the function. This library provides several methods for function optimization.

% Here's a Python code snippet that defines the function and uses the scipy.optimize.minimize function to find its minimum within the given bounds:

% python
% Copy code
% import numpy as np
% from scipy.optimize import minimize

% # Define the function
% def f(x, r, R):
%     h, H = x
%     return (R**2 * H**2 + 2 * r**2 * h**2) / (R**2 * H + 4 * r**2 * h)

% # Define the bounds and initial guess
% bounds = [(1, 3), (1, 5)]
% x0 = [2, 3]  # initial guess

% # Define the parameters r and R
% r = 0.1  # replace with the actual value
% R = 1.0  # replace with the actual value

% # Find the minimum of the function
% res = minimize(f, x0, args=(r, R), bounds=bounds)

% print("The minimum of the function is at h = {:.2f} cm, H = {:.2f} cm".format(*res.x))
% In this code, x0 is the initial guess for the values of h and H. The bounds variable defines the lower and upper bounds for h and H. The args parameter of the minimize function is used to pass the parameters r and R to the function f. The result of the minimize function is an object that contains information about the optimization result, including the values of h and H at the minimum (res.x).

% Please replace r and R with the actual values for the radius of the legs and the table top, respectively.
%     \end{lstlisting}
%     \item User:
%     \begin{lstlisting}
%         Which optimization method does minimize use?
%     \end{lstlisting}
%     \begin{lstlisting}
%     \item GPT:
%     The scipy.optimize.minimize function in Python uses the Broyden–Fletcher–Goldfarb–Shanno (BFGS) algorithm by default for unconstrained problems. The BFGS method is a quasi-Newton method that uses function values and gradients to build up a picture of the surface to be optimized.

% However, when bounds are provided (as in your case), minimize defaults to the Limited-memory BFGS (L-BFGS-B) method. The L-BFGS-B method is a modification of the BFGS method that is more suitable for problems with many variables and constraints on the variable values.

% The method to be used can be specified using the method parameter of the minimize function. Other methods available include 'Nelder-Mead', 'Powell', 'CG', 'TNC', 'COBYLA', 'SLSQP', and others. The choice of method depends on the nature of the problem (e.g., whether it's constrained, whether the function is smooth, whether gradients are available, etc.).
% \end{lstlisting}
%     \item User: 
%     \begin{lstlisting}
%         What do you think is the best choice here?
%     \end{lstlisting}
%     \item GPT:
%     \begin{lstlisting}
%         Given that we have bounds on the variables, the Limited-memory BFGS (L-BFGS-B) method is a good choice for this problem. L-BFGS-B is an optimization algorithm in the family of quasi-Newton methods that approximates the Broyden–Fletcher–Goldfarb–Shanno (BFGS) algorithm using a limited amount of computer memory. It's a popular choice for optimization problems where there are constraints on the parameters.

% The L-BFGS-B method is particularly suitable for high-dimensional problems, and it can handle the bounds on the parameters efficiently. It also doesn't require the computation of the second derivatives (the Hessian matrix), which can be computationally expensive for complex functions.

% Therefore, using the L-BFGS-B method with the scipy.optimize.minimize function, as in the provided Python code, would be a good approach for finding the minimum of the function within the given bounds.
%     \end{lstlisting}
%     \item User:
%     \begin{lstlisting}
%         Can you compute expressions for the gradients of this problem, and provide code that uses them to accelerate the L-BFGS-B call?
%     \end{lstlisting}
%     \item GPT:
%     \begin{lstlisting}
%         Sure, the gradient of a function is a vector of its partial derivatives with respect to each of the variables. In this case, the gradient of the function 
% �
% (
% ℎ
% ,
% �
% )
% =
% �
% 2
% �
% 2
% +
% 2
% �
% 2
% ℎ
% 2
% �
% 2
% �
% +
% 4
% �
% 2
% ℎ
% f(h,H)= 
% R 
% 2
%  H+4r 
% 2
%  h
% R 
% 2
%  H 
% 2
%  +2r 
% 2
%  h 
% 2
 
% ​
%   is a vector with two components: the partial derivative with respect to 
% ℎ
% h and the partial derivative with respect to 
% �
% H.

% Let's compute these partial derivatives:

% ∂
% �
% ∂
% ℎ
% =
% 4
% �
% 2
% ℎ
% (
% �
% 2
% �
% +
% 4
% �
% 2
% ℎ
% )
% −
% 2
% �
% 2
% ℎ
% 2
% (
% 4
% �
% 2
% )
% (
% �
% 2
% �
% +
% 4
% �
% 2
% ℎ
% )
% 2
% ∂h
% ∂f
% ​
%  = 
% (R 
% 2
%  H+4r 
% 2
%  h) 
% 2
 
% 4r 
% 2
%  h(R 
% 2
%  H+4r 
% 2
%  h)−2r 
% 2
%  h 
% 2
%  (4r 
% 2
%  )
% ​
 
% ∂
% �
% ∂
% �
% =
% 2
% �
% 2
% �
% (
% �
% 2
% �
% +
% 4
% �
% 2
% ℎ
% )
% −
% �
% 2
% �
% 2
% (
% �
% 2
% )
% (
% �
% 2
% �
% +
% 4
% �
% 2
% ℎ
% )
% 2
% ∂H
% ∂f
% ​
%  = 
% (R 
% 2
%  H+4r 
% 2
%  h) 
% 2
 
% 2R 
% 2
%  H(R 
% 2
%  H+4r 
% 2
%  h)−R 
% 2
%  H 
% 2
%  (R 
% 2
%  )

 
% We can then provide these gradients to the minimize function to accelerate the optimization process. Here's the updated Python code:

% python
% Copy code
% import numpy as np
% from scipy.optimize import minimize

% # Define the function
% def f(x, r, R):
%     h, H = x
%     return (R**2 * H**2 + 2 * r**2 * h**2) / (R**2 * H + 4 * r**2 * h)

% # Define the gradient of the function
% def grad_f(x, r, R):
%     h, H = x
%     dfdh = (4 * r**2 * h * (R**2 * H + 4 * r**2 * h) - 2 * r**2 * h**2 * (4 * r**2)) / (R**2 * H + 4 * r**2 * h)**2
%     dfdH = (2 * R**2 * H * (R**2 * H + 4 * r**2 * h) - R**2 * H**2 * (R**2)) / (R**2 * H + 4 * r**2 * h)**2
%     return np.array([dfdh, dfdH])

% # Define the bounds and initial guess
% bounds = [(1, 3), (1, 5)]
% x0 = [2, 3]  # initial guess

% # Define the parameters r and R
% r = 0.1  # replace with the actual value
% R = 1.0  # replace with the actual value

% # Find the minimum of the function
% res = minimize(f, x0, args=(r, R), jac=grad_f, bounds=bounds)

% print("The minimum of the function is at h = {:.2f} cm, H = {:.2f} cm".format(*res.x))
% In this code, jac=grad_f tells minimize to use the function grad_f to compute the gradient of the function at each step. This can significantly speed up the optimization process, especially for complex functions or large problems.
%     \end{lstlisting}
% \end{enumerate}

In later sections, we will demonstrate how GPT struggles to solve a (much) more difficult version of this optimization problem.

There is one more pitfall.  If users do not prompt GPT to explicitly show its work, it may resort to ``common-sense'' reasoning about a problem.  Although this could be correct, it provides no certificate to a user.  GPT does just that, in an alternate second query in this chain, showin in Listing TODO.

\iffalse

\begin{enumerate}
    \item User:
    \begin{lstlisting}
         Ok.  Let's say the bounds for the height of the legs are between 1cm and 3 cm, and the height of the table is between 1 and 5 cm.  Please optimize the parameters such that the table is as statically stable as possible, and explain the process.
    \end{lstlisting}
    \item GPT:    
    \begin{lstlisting}
   
ChatGPT
The static stability of a table is primarily determined by its center of mass and the area of its base. A table is more stable if its center of mass is lower and the area of its base is larger.

In this case, the table's base is defined by the placement of the four legs. If we assume that the legs are placed at the maximum radius from the center of the table, the base area is maximized and thus the stability is also maximized.

The center of mass is determined by the heights of the table top and the legs. To lower the center of mass, we want to minimize the height of the table top and maximize the height of the legs.

Given the bounds you provided, the optimal parameters for the table would be:

Height of the legs (h): 3 cm
Height of the table top (H): 1 cm
This configuration maximizes the height of the legs and minimizes the height of the table top, thus lowering the center of mass and increasing the table's static stability.

Please note that this analysis assumes that the table is on a flat surface and that the weight distribution in the table top is uniform. If the weight distribution is not uniform (for example, if there is a heavy object on one side of the table), the table may still tip over.

Also, this analysis does not take into account the dynamic stability of the table, which involves how the table responds to forces and movements. For example, a table with very tall, thin legs may be statically stable but not dynamically stable.

Finally, this analysis assumes that the table is made of a uniform material. If the table top is made of a heavier material than the legs, the center of mass will be higher and the table will be less stable.
    \end{lstlisting}
\end{enumerate}
\fi

There are problems in which the usual pitfalls regarding GPT arise --- if it is difficult to find a library to solve a particular task, it might give up or try writing its own code; if the code is detail-heavy, it may be too difficult for GPT to write correctly and the solution may be incorrect; if a library does exist but it is uncommonly used, it may give incorrect instructions on how to install that library; or, in some cases, it may hallucinate a library.


TODO: Add renders

\paragraph{ \textbf{Q1.2} Can GPT reason about different problem types and choose a correct solver? }

GPT manages to be extremely robust in reasoning about problems and choosing an adequate solver for that problem.  In cases where a more sophisticated algorithm was needed, it tended to choose at least the correct algorithm class, but was not always aware of the best version or implementation.  A notable example is in optimizing robot topologies for ground locomotion, where GPT identified an evolutionary algorithm as an effective optimization method, but did not choose any state-of-the-art specific algorithms or implementations.

Below we highlight some different classes of problems:

TODO:
Format as: Name, Search Space, Constraint Space, Objective Space, Other considerations, Chosen optimization method.

-Robot Arm optimization - Continuous Search Space, Reachability (continuous) constraint, Continuous Objective, 2nd order gradient-based optimization.

-Robot topology design - Graph-search space, No constraints, objective continuous, TODO, Evolution optimization method

-Printing Parameters - Continuous search space, bound constraints, objective continuous, very expensive evaluation function, Bayesian Optimization

-Multicopter Optimization - Continuous search space, bound constraints, objective continuous, requires simulation in the loop and knowledge of quadcopter materials, Grid Search

-Mixed Optimization?  Bookshelf. TODO

-Logical Constraints, continuous objective --- Robot motion planning TODO


TODO: Add renders

\begin{figure}[ht]
\begin{subfigure}[t]{0.5\linewidth}
  \centering
  \includegraphics[width=0.4\linewidth]{figures/cabinet_init.png}
  \caption{Initial Cabinet Design}
\end{subfigure}%
\begin{subfigure}[t]{0.5\linewidth}
  \centering
  \includegraphics[width=0.4\linewidth]{figures/cabinet_opt_5000.png}
  \caption{Optimized Cabinet with Volume Constraint}
\end{subfigure}
\caption{\textbf{Single Objective with Constraint Optimization.} \textbf{Left:} A cabinet with initial height, width, and depth of 55 in. \textbf{Right:} Using an off-the-shelf solver provided by scipy.optimize, \gpt provides a Python script that optimizes the cabinet's height, width, and depth given a desired volume while minimizing the material cost. We show a cabinet that meets the volume constraint of 5000 cubic inches of storage capacity.}
\label{fig:cabinet_opt_render}
\end{figure}


\subsection{Can this tool support optimization in contexts that require additional knowledge?}

In some cases, non-expert, and even some expert users may find that a given inverse design problem has nuances that they have not considered.  In this section, we examine how LLMs can help less experienced users to specify and navigate inverse design problems.  Further, we demonstrate the ability of LLMs to aid in generating design specifications that are difficult to specify or quantify mathematically.



\textbf{2.1} Can GPT assist designers in navigating the landscape of possible trade-offs when multiple conflicting objectives are present?

Listing TODO shows the design process of a chair.  The first query demonstrates the breadth of knowledge of GPT in design considerations, as GPT proposes a list of facets one must care about in furniture construction.  From that list, the user chooses two design criteria, and asks GPT to generate a parameterized chair design by selecting important design parameters as well creating a parameterized template.  When asked how to optimize for both design parameters (without hinting at the need for tradeoffs), GPT informs the user that this is a multi-objective design problem, and suggests a common algorithm for multi-objective optimization (NSGA-II).  A Pareto Front of ``optimal'' chair designs for the parameters found from running the algorithm can be found in Fig. TODO.


\textbf{2.2} Can GPT support design exploration and optimization when the design 
space is not properly defined or fully bounded?

The previous chair example similarly demonstrates the ability for GPT to recommend reasonable parameters for a design without needing to be manually prompted by a user, applying its knowledge of the target domain.  Here, a user simply asks for ``parameters''; GPT (reasonably) offers continuous parameterizations of a typical chair (and provides a 3D model on request) and offers reasonable ranges without neededing to be prompted.  While discrete parameters are possible with a chair, they are less likely to have a significant impact than its raw dimensions, and most chairs are comprised specifically of four legs, a seat, and a back. 

This cannot translate to completely novel problems, but it can apply knowledge of aspects of a problem to new problems in familiar domains.  Listing TODO shows an example of a new type of GPT helping to design a novel machine invented by a user; since it is synthesized from existing ideas, GPT can use its knowledge of those preexisting domains and their components to recommend reasonable design parameter ranges. 

\textbf{2.3} Can GPT support design optimization when objectives are not easily quantifiable?

Some objectives, typically those requiring human feedback and opinion, are difficult to specify as a mathematical objective; in those cases, a numerical optimization approach is intractable.  One solution sometimes employed is to train a surrogate model of user opinions (TODO: cite); however, as GPT is a large language model that encodes human knowledge, it is reasonable to wonder if GPT can aid in directly modifying designs for high level objectives.

Listing TODO presents an example of CLIP (TODO: cite) being used to steer the design process.  Starting with a base design for a cabinet, the user asks GPT to alter the design stylistically, \textit{e.g.} to make it look ``Mid-Century Modern'' or ``Egyptian'' styled.  GPT provides new designs to try to match those styles.  We use CLIP as feedback on renders of the designs to determine if they have become more or less like the style requested.  Figure TODO: shows the evolution of designs through this process, with the prompts displayed in Listing TODO.  As can be seen, the fidelity of designs generated through this process is low, and G

\iffalse
-GPT has the ability to do basic math.
-That math is not always error-proof.
-In addition, it has the ability to resort to two other tools at its disposal: a) Plugins, b) Code that can be run by a user (or by a program calling into GPT).
-Each of these approaches has certain pitfalls, as we discuss

P1: The Table example.
-Setup the problem
-Why is this straightforward?
-An intuitive answer exists
-GPT finds the intuitive answer.

-Approach 1: Wolfram Alpha
-The problem: Timeout

-Approach 2: GPT's own math
-The problem: Reasoning is not super robust about complex algebra.
-As we'll see, GPT's internal calculus is also limited by the fact that it can make mistakes, somethign that will rear its head in the section TODO.



P2: The arm example (code)

\fi

\iffalse
% Robot arm reaching a target location 
% Plan to move a robot arm to reach a location
% Cabinet 


- propose modifications of a single design (no need to create a design space) (capacitor examples)
- create from library 
( drone example) 


The remainder of this section begins by walking through a simple end-to-end example.  We then examine a number of questions regarding the capabilities of LLMs.  For each of these questions, we aim to determine what LLMs are currently capable of, and what still seems to be beyond their capabilities.


\subsection{A Simple Example}
A general effective strategy for optimizing designs is to begin by asking for a \textit{forward model} of the problem, and then asking for a means for searching over that forward model in order to solve the \textit{inverse problem}.  This first query can include detailed information about the design space and/or the performance space, but the user can in some cases trust the LLM to define these reasonably.

Listing TODO shows a very simple example of optimizing over a two-linked robot arm, for a reachability task.  The first query creates the model.  In the second query, the LLM chooses to optimize the geometry over LLM, constrained on the task constraints, using L-BFGS, a constrained gradient-based second-order optimizer.  Following this example, we show demonstrations of inserting priors of design and performance metrics.


\iffalse
User:
\begin{lstlisting}
    I'm trying to design a robot arm that can move its end effector directly vertically half a meter.  Can you help by providing a design for such a robot?  It should only use rotational motors.  I need to know the morphology of the robot - the dimensions of the links, and how they are connected.  Or, if you don't know the dimensions or the morphology, you can provide code to search for dimensions that would work for the task (through simulation).
\end{lstlisting}
GPT:
\begin{lstlisting}
import numpy as np

# Set the desired vertical distance
d = 0.5  # 0.5 meters

# Set the initial length of the arm links (randomly or based on prior knowledge)
l1 = 0.25  # 0.25 meters
l2 = 0.25  # 0.25 meters

# Calculate the angles using inverse kinematics
theta2 = np.arccos((d**2 - l1**2 - l2**2) / (2 * l1 * l2))
theta1 = np.arctan2(l2 * np.sin(theta2), l1 + l2 * np.cos(theta2))

# Confirm that the end effector reaches the desired position
x = l1 * np.cos(theta1) + l2 * np.cos(theta1 + theta2)
y = l1 * np.sin(theta1) + l2 * np.sin(theta1 + theta2)

print("The end effector is at position: ", (x, y))

# Now you can run a loop to iterate over various lengths for l1 and l2
# within a feasible range and see which combination gives you the best result.
# You would have to define "best" - could be smallest, lightest, simplest, etc.
\end{lstlisting}

User:
\begin{lstlisting}
    Can you write the code for that parameter search?
\end{lstlisting}

GPT:
\begin{lstlisting}
    import numpy as np
from scipy.optimize import minimize

# Set the desired vertical distance
d = 0.5  # 0.5 meters

# Define the objective function (the function to minimize)
def objective(x):
    return x[0] + x[1]

# Define the constraint (the robot arm must reach the desired height)
def constraint(x):
    l1, l2 = x[0], x[1]
    
    theta2 = np.arccos((d**2 - l1**2 - l2**2) / (2 * l1 * l2))
    theta1 = np.arctan2(l2 * np.sin(theta2), l1 + l2 * np.cos(theta2))
    
    y = l1 * np.sin(theta1) + l2 * np.sin(theta1 + theta2)
    
    # The constraint function must return a value greater than 0 for feasible solutions
    return y - d

# Define the initial guess for the lengths
x0 = np.array([0.25, 0.25])

# Define the bounds for the lengths (in this case, each link must be between 0.1 and 0.5 meters long)
bnds = [(0.1, 0.5), (0.1, 0.5)]

# Define the constraint dictionary
con = {'type': 'ineq', 'fun': constraint}

# Solve the optimization problem
solution = minimize(objective, x0, bounds=bnds, constraints=con)

print("The optimal lengths are: ", solution.x)
\end{lstlisting}
\fi
\
Here, GPT created the specified constraint and chose the design space (including parameter bounds) and a performance metric, and chose an adequate optimization method that's easily accessible from Python.  We do note that GPT did not provide gradient information about any of the objectives or constraints, which would help accelerate the search.

Listing TODO refines the above example to include these aspects.
\iffalse

User:
\begin{lstlisting}
Scipy's minimize defaults go L-BFGS.  That can use gradient information.  Can you provide code for the gradient computation and update the example to use that?
\end{lstlisting}

GPT: (TODO: check correctness)
\begin{lstlisting}
    import numpy as np
from scipy.optimize import minimize

# Set the desired vertical distance
d = 0.5  # 0.5 meters

# Define the objective function (the function to minimize)
def objective(x):
    return np.sum(x)

# Gradient of the objective function
def grad_objective(x):
    return np.array([1.0, 1.0])

# Define the constraint (the robot arm must reach the desired height)
def constraint(x):
    l1, l2 = x[0], x[1]
    
    theta2 = np.arccos((d**2 - l1**2 - l2**2) / (2 * l1 * l2))
    theta1 = np.arctan2(l2 * np.sin(theta2), l1 + l2 * np.cos(theta2))
    
    y = l1 * np.sin(theta1) + l2 * np.sin(theta1 + theta2)
    
    # The constraint function must return a value greater than 0 for feasible solutions
    return y - d

# Gradient of the constraint
def grad_constraint(x):
    l1, l2 = x[0], x[1]
    
    theta2 = np.arccos((d**2 - l1**2 - l2**2) / (2 * l1 * l2))
    theta1 = np.arctan2(l2 * np.sin(theta2), l1 + l2 * np.cos(theta2))
    
    dtheta2_dl1 = -(l1 + l2 * np.cos(theta2)) / (l1 * l2 * np.sqrt(1 - ((d**2 - l1**2 - l2**2) / (2 * l1 * l2))**2))
    dtheta2_dl2 = -(l1 + l2 * np.cos(theta2)) / (l1 * l2 * np.sqrt(1 - ((d**2 - l1**2 - l2**2) / (2 * l1 * l2))**2))
    
    dtheta1_dl1 = (l2 * np.cos(theta2) * dtheta2_dl1 - (l1 + l2 * np.cos(theta2))) / (l1**2 + l2**2 + 2*l1*l2*np.cos(theta2))
    dtheta1_dl2 = (l2 * np.cos(theta2) * dtheta2_dl2 - (l1 + l2 * np.cos(theta2))) / (l1**2 + l2**2 + 2*l1*l2*np.cos(theta2))
    
    dy_dl1 = np.sin(theta1) - l1 * np.cos(theta1) * dtheta1_dl1 + np.sin(theta1 + theta2) * (dtheta1_dl1 + dtheta2_dl1)
    dy_dl2 = np.sin(theta1 + theta2) * (dtheta1_dl2 + dtheta2_dl2)
    
    return np.array([dy_dl1, dy_dl2])

# Define the initial guess for the lengths
x0 = np.array([0.25, 0.25])

# Define the bounds for the lengths (in this case, each link must be between 0.1 and 0.5 meters long)
bnds = [(0.1, 0.5), (0.1, 0.5)]

# Define the constraint dictionary
con = {'type': 'ineq', 'fun': constraint, 'jac': grad_constraint}

# Define the options for the solver
options = {'disp': True, 'iprint': 1, 'eps': 1.4901161193847656e-08}

# Solve the optimization problem
solution = minimize(objective, x0, jac=grad_objective, bounds=bnds, constraints=con, method='L-BFGS-B', options=options)

print("The optimal lengths are: ", solution.x)
\end{lstlisting}


User:
\begin{lstlisting}
Let's say we wanted to make the objective function something else, something related to the configuration space.  Specifically, we want to find a design such that the joint connecting the two links is as "straight" as possible when it reaches its target point with its end effector.  How would we modify the code to do that?
\end{lstlisting}

GPT (TODO: check correctness):
\begin{lstlisting}
    import numpy as np
from scipy.optimize import minimize

# Set the desired vertical distance
d = 0.5  # 0.5 meters

# Define the objective function (the function to minimize)
def objective(x):
    l1, l2 = x[0], x[1]
    
    theta2 = np.arccos((d**2 - l1**2 - l2**2) / (2 * l1 * l2))
    
    return (theta2 - np.pi)**2

# Gradient of the objective function
def grad_objective(x):
    l1, l2 = x[0], x[1]
    
    theta2 = np.arccos((d**2 - l1**2 - l2**2) / (2 * l1 * l2))
    
    dtheta2_dl1 = -(l1 + l2 * np.cos(theta2)) / (l1 * l2 * np.sqrt(1 - ((d**2 - l1**2 - l2**2) / (2 * l1 * l2))**2))
    dtheta2_dl2 = -(l1 + l2 * np.cos(theta2)) / (l1 * l2 * np.sqrt(1 - ((d**2 - l1**2 - l2**2) / (2 * l1 * l2))**2))
    
    d_obj_dl1 = 2 * (theta2 - np.pi) * dtheta2_dl1
    d_obj_dl2 = 2 * (theta2 - np.pi) * dtheta2_dl2
    
    return np.array([d_obj_dl1, d_obj_dl2])

# Define the constraint (the robot arm must reach the desired height)
# The same as before...

# Gradient of the constraint
# The same as before...

# Define the initial guess for the lengths
x0 = np.array([0.25, 0.25])

# Define the bounds for the lengths (in this case, each link must be between 0.1 and 0.5 meters long)
bnds = [(0.1, 0.5), (0.1, 0.5)]

# Define the constraint dictionary
con = {'type': 'ineq', 'fun': constraint, 'jac': grad_constraint}

# Define the options for the solver
options = {'disp': True, 'iprint': 1, 'eps': 1.4901161193847656e-08}

# Solve the optimization problem
solution = minimize(objective, x0, jac=grad_objective, bounds=bnds, constraints=con, method='L-BFGS-B', options=options)

print("The optimal lengths are: ", solution.x)
\end{lstlisting}

User:
\begin{lstlisting}
I'm not sure how we know if these are good parameter bounds.  Can you provide a systematic way for choosing them, or a principled justification for bounds you choose?  Please provide new bounds and concrete reasoning about why these are the maximum and minimum, and why going beyond them would not help our optimization problem find any better results.  Also, please choose an initial guess for the decision vector and explain why it is a good choice.  This for the problem in which we want to reach a target of 0.5 vertically with the end-effector.
\end{lstlisting}

\begin{lstlisting}
The selection of the parameter bounds and initial guess is often driven by practical constraints and prior knowledge about the problem.

In the context of this robot arm design problem, here are some aspects to consider when defining the bounds and initial guess:

Bounds

Physical constraints: The length of the robot arm's links cannot be negative or zero, so the lower bound must be greater than zero. On the other hand, the upper bound may be limited by factors such as the materials used to construct the arm, the strength of the motors, and the size of the workspace. For instance, an excessively long arm might be too heavy for the motors to move, or it might be too large to fit in the intended workspace.

Reachability constraints: The robot arm must be able to reach the desired vertical distance. The sum of the lengths of the links should be at least equal to this distance. This provides a lower bound for the sum of l1 and l2.

Given the target distance of 0.5 meters, we can refine the bounds as follows:

Lower bound: To ensure that the arm can reach the target, each link should be at least 0.25 meters long if we consider a straight line reach scenario. A smaller value could still be feasible if we allow the arm to bend, but 0.25 meters is a conservative lower bound.

Upper bound: This depends on the practical constraints mentioned earlier, but let's say we limit each link to 1 meter. This would allow for a straight reach to targets up to 2 meters away, which seems reasonable for a desktop or industrial robot arm.

These bounds are (0.25, 1) for both l1 and l2.

Initial Guess

The initial guess can influence the speed and success of the optimization. It's typically chosen based on prior knowledge or assumptions about the problem.

In this case, a reasonable initial guess could be to set both l1 and l2 to 0.5, which would allow the arm to reach the target in a straight line. This seems like a good starting point because it satisfies the reachability constraint and is within the defined bounds.

Here's how you would define the bounds and initial guess:

python
Copy code
# Define the bounds for the lengths
bnds = [(0.25, 1), (0.25, 1)]

# Define the initial guess for the lengths
x0 = np.array([0.5, 0.5])
These values should provide a good balance between ensuring feasibility (the arm can reach the target) and leaving room for the optimization to find a better solution (the arm's joint is as straight as possible). However, keep in mind that the effectiveness of these choices may depend on the specifics of the robot arm and the target.
\end{lstlisting}

\fi



\subsection{Major Questions}


\paragraph{ \textbf{Q1} Can GPT identify optimal designs when a design space and performance metric are provided? }
 
TODO:

-Yes, walk through the example above, and the zoo, and summarize.

When is GPT unable to give reasonable recommendations?
a) If anything, it tends to be extra conservative (give examples).
b) When it has a bad sense of scale of the problem.  This is especially true in novel problems, or when dealing with somewhat abstract problems


\paragraph{\textbf{Q2} Can GPT assist designers in navigating the landscape of possible trade-offs when multiple conflicting objectives are present?}

TODO

\paragraph{ \textbf{Q3} Can GPT support design exploration and optimization when the design space is not properly defined or fully bounded?}

Yes.  In many cases, ChatGPT will actually ``fill in'' or autocomplete objectives and constraints.

Motivators: Table - automatically chose certain variables to be constant when it ran into issues.  Robot reaching example (chose an objective and a constraint).


\paragraph{\textbf{Q4} Can GPT support design optimization when objectives are not easily quantifiable?}

TODO: Unclear.

\paragraph{\textbf{Q5} Can GPT choose reasonable algorithms for different types of supports for constraints, objectives, and decision spaces (\textit{e.g.} continuous, discrete, binary, \textit{etc.}}

Yes.  See the Zoo.

When does it fail?  If anything, it doesn't always have knowledge about some of the state-of-the-art methods.  It tends to almost always recommend scipy's minimize (sometimes smartly selecting the algorithm), and sometimes provides its own, more naive implementations of other methods (such as evolutionary algorithms).  TODO: Does using the Bing Plugin help with this?

\textbf{Q6} When can GPT solve a problem analytically, and when does it need to resort to using an outside tool? (\textit{i.e.} a programmed algorithm).  And, when does it fail?

a) If there is a common-sense solution (table example, or the robot arm).

b) When it is a straightforward Analysis problem where the gradients tend to exist --- but in this case, it also is sometimes overly confident about its domain knowledge and will provide wrong information (TODO: show the quadcopter).

c) When it can make a call to a tool like Wolfram Alpha and it isn't too difficult in complexity

Failure case: Cannot create an analytical/evaluation model (e.g. FEM) or when it hallucinates libraries.


\subsection{The Zoo}
Below we show some demonstrations of inverse design methods used by LLMs.

TODO:
To add: 
1. Evolutionary algorithm for robot topology search.

2. Baysian Optimization for Printing Parameters

3. Table example




\subsubsection{Optimizing Cabinet Design w.r.t. Constraint}

We investigate whether GPT can output a reasonable cost function and design that optimizes the function when provided an example design, a parameterization of the design space, and a text description of the objective. One instantiation of this problem setting is with furniture: can GPT optimize the design of a cabinet such that the result has a user-specified volume while minimizing the cost to build it? First, we prompt \gpt with an example cabinet design in OpenSCAD and a parameterization of the design, which includes bounds for the parameters, and ask it to generate the functions to compute volume and material cost. Once the user verifies the accuracy of the functions, we have \gpt  output a python script that can minimize the cabinet's material cost with respect to a given volume constraint. The resulting code is shown in Fig. \ref{fig:cabinet_opt} and an example of an optimized cabinet is shown in Fig. \ref{fig:cabinet_opt_render}.

\begin{figure}[h]
\begin{chat}{false} % param: prevent page breaks in chat (true=page breaks allowed, false=not allowed)

\begin{userprompt}{0.0\textwidth}{} 
Assume that you can call the below functions.
\begin{gptcodeblock}{Python}
def compute_storage_capacity(cabinet_height, cabinet_width, cabinet_depth, board_thickness):
    """
    This function calculates the storage capacity of the cabinet.
    """
    # ...implementation omitted for brevity...
    return storage_capacity

def compute_material_cost(cabinet_height, cabinet_width, cabinet_depth, board_thickness, cost_per_cubic_inch):
    """
    This function calculates the material cost of the cabinet.
    """
    # ...implementation omitted for brevity...
    return material_cost
\end{gptcodeblock}

In addition, a cabinet design can be parameterized as follows. The bounds of each parameter is specified along with rationale for these bounds.

\begin{itemize}
    \item boardThickness: (0.1, 5) inches. The board thickness should be positive and typically not exceed 5 inches for a cabinet of this size. It's also unlikely to be less than 0.1 inches due to structural stability concerns.
    \item cabinetHeight, cabinetWidth, cabinetDepth: (10, 100) inches. These dimensions should be positive and typically fall within a reasonable range for a cabinet. The exact bounds will depend on the specific use case and available space.
    \item ...parameters omitted for brevity...
\end{itemize}

Write a script to find the cabinet of the correct volume that minimizes cost using any library you want. If the volume constraint is not satisfied, specify this. Assume that the cost per cubic inch of the materials, the board thickness, and the volume constraint will be user specified. Demonstrate that the script works with example user specifications.

\end{userprompt}

\begin{gptresponse}{0.0\textwidth}{} ...text omitted for brevity...
\begin{gptcodeblock}{Python}
from scipy.optimize import minimize

# Set some example values
desired_volume = 1000  # Desired storage capacity in cubic inches
cost_per_cubic_inch = 0.05  # Cost per cubic inch of the material
board_thickness = 0.5  # Thickness of the board

def objective_function(x):
    """
    Define the function to be minimized, in this case the cost of the cabinet material.
    """
    cabinet_height, cabinet_width, cabinet_depth = x  # Extract cabinet dimensions
    return compute_material_cost(cabinet_height, cabinet_width, cabinet_depth, board_thickness, cost_per_cubic_inch)

def constraint_function(x):
    """
    Define the function to represent the constraint, in this case the desired volume.
    """
    cabinet_height, cabinet_width, cabinet_depth = x  # Extract cabinet dimensions
    volume = compute_storage_capacity(cabinet_height, cabinet_width, cabinet_depth, board_thickness)
    return volume - desired_volume  # This should be equal to zero when the desired volume is met

# Initial guess (start at the mid-point of the possible range for each dimension)
x0 = [55, 55, 55]

# Define bounds for each dimension
bounds = [(10, 100), (10, 100), (10, 100)]  # Lower and upper bound for each dimension

# Define the constraints
constraints = [{'type': 'eq', 'fun': constraint_function}]

# Call the optimizer
result = minimize(objective_function, x0, method='SLSQP', bounds=bounds, constraints=constraints)

# Print the result
if result.success:
    print(f"Optimized cabinet dimensions: {result.x}")
    print(f"Minimum cost: {result.fun}")
else:
    print(f"Optimization failed with message: {result.message}")

    \end{gptcodeblock}
\end{gptresponse}
\end{chat}
\caption{\label{fig:cabinet_opt} The performance and cost functions are generated by prompting \gpt. To find the minimum of the material cost function with respect to volume, \gpt calls scipy.optimize's minimize function with an appropriate solver. In addition, the provided code extracts the relevant bounds and a suitable initial guess from the prompt and checks whether or not the optimization was successful. }
\end{figure}
% \begin{figure}[h]
% \begin{chat}{false}
%     \begin{gptresponse}{0.0\textwidth}{} ...text omitted for brevity...
% \begin{gptcodeblock}{Python}
% from scipy.optimize import minimize

% # Set some example values
% desired_volume = 1000  # Desired storage capacity in cubic inches
% cost_per_cubic_inch = 0.05  # Cost per cubic inch of the material
% board_thickness = 0.5  # Thickness of the board

% def objective_function(x):
%     """
%     Define the function to be minimized, in this case the cost of the cabinet material.
%     """
%     cabinet_height, cabinet_width, cabinet_depth = x  # Extract cabinet dimensions
%     return compute_material_cost(cabinet_height, cabinet_width, cabinet_depth, board_thickness, cost_per_cubic_inch)

% def constraint_function(x):
%     """
%     Define the function to represent the constraint, in this case the desired volume.
%     """
%     cabinet_height, cabinet_width, cabinet_depth = x  # Extract cabinet dimensions
%     volume = compute_storage_capacity(cabinet_height, cabinet_width, cabinet_depth, board_thickness)
%     return volume - desired_volume  # This should be equal to zero when the desired volume is met

% # Initial guess (start at the mid-point of the possible range for each dimension)
% x0 = [55, 55, 55]

% # Define bounds for each dimension
% bounds = [(10, 100), (10, 100), (10, 100)]  # Lower and upper bound for each dimension

% # Define the constraints
% constraints = [{'type': 'eq', 'fun': constraint_function}]

% # Call the optimizer
% result = minimize(objective_function, x0, method='SLSQP', bounds=bounds, constraints=constraints)

% # Print the result
% if result.success:
%     print(f"Optimized cabinet dimensions: {result.x}")
%     print(f"Minimum cost: {result.fun}")
% else:
%     print(f"Optimization failed with message: {result.message}")

%     \end{gptcodeblock}
% \end{gptresponse}
% \end{chat}
% \caption{\label{fig:cabinet_opt}To find the minimum of the material cost function with respect to volume, \gpt calls scipy.optimize's minimize function with an appropriate solver. In addition, the provided code extracts the relevant bounds and a suitable initial guess from the prompt and checks whether or not the optimization was successful.}
% \end{figure}

% GPT is able to output reasonable functions computing the storage capacity and material cost, though there was an error in computing shelf volume. 

\subsubsection{Planning for Robot Manipulation}

We now study a planning problem, where given a claw attached to an arm and an environment with objects and bins, \gpt must control the arm-claw robot with a sequence of commands that picks up all objects and places them into bins. We present an interface for the arm-claw such that the physical embodiment of the arm-claw robot does not matter, allowing \gpt to simply reason about the movement of the claw and whether the claw should grasp or release an object. Due to the nature of the problem, an important constraint is that the claw must visit an object to pick it up before dropping it off at a bin. Another is that a bin can only hold one object. While formalizing the constraint that the claw must visit an object before a bin is not a trivial task, the performance objective is minimizing the distance that the claw travel. To simplify the problem, we also add that the maximum number of objects and bins is 3 each, making brute force a valid solution. The initial prompt and result is shown in Fig. \ref{fig:claw1}.

\begin{figure}[h]
\begin{chat}{false} % param: prevent page breaks in chat (true=page breaks allowed, false=not allowed)

\begin{userprompt}{0.0\textwidth}{} 
You are tasked with controlling an arm and a claw. The goal is to pick up an object on the ground with the claw and place it in a bin large enough for the object to fit in. You are working with (x, y, z) coordinates where 0 <= x, y, z <= 50. Below are functions you can use to control the arm and claw. 
Arm: 	
\begin{itemize}
    \item translate\_x(x\_dist): Translates the claw in the x direction by x\_dist.
    \item translate\_y(y\_dist): Translates the claw in the y direction by y\_dist.
    \item translate\_z(z\_dist): Translates the claw in the z direction by z\_dist. 
\end{itemize}

Claw: 	
\begin{itemize}
    \item grasp(): If there is an object at the claw's current location, the object will be grasped. When the object is grasped and the claw is moved, the object is moved to the same location as the claw's fingertips. 	
    \item release(): If the claw is grasping an object, the object will fall to the ground directly underneath it at z=0 or to any bin directly underneath it. 
\end{itemize}

...additional specifications omitted  for brevity...
\end{userprompt}

\begin{gptresponse}{0.0\textwidth}{} 
    ...text omitted for brevity...
    \begin{gptcodeblock}{Python}
import math

def move_arm(claw_initial, objects_initial, bins, T_max):
    def distance(p1, p2):
        # Calculate Euclidean distance between two points
        return math.sqrt((p1[0] - p2[0])**2 + (p1[1] - p2[1])**2 + (p1[2] - p2[2])**2)
    
    actions = []
    power_used = 0
    claw_current = list(claw_initial)

    while objects_initial and power_used <= T_max:
        # Find nearest object
        nearest_object = min(objects_initial, key=lambda o: distance(claw_current, o))

        # Calculate necessary translations to reach the object
        translations = [o - c for o, c in zip(nearest_object, claw_current)]

        # Check if there's enough power left to reach the object and drop it in a bin
        if power_used + sum(abs(t) for t in translations) * 2 > T_max:
            break

        # Move to the object
        actions.append(('translate_x', translations[0]))
        actions.append(('translate_y', translations[1]))
        actions.append(('translate_z', translations[2]))
        actions.append(('grasp',))

        # Update claw position and power used
        claw_current = nearest_object
        power_used += sum(abs(t) for t in translations)

        # Find nearest bin
        nearest_bin = min(bins, key=lambda b: distance(claw_current, b))

        # Calculate necessary translations to reach the bin
        translations = [b - c for b, c in zip(nearest_bin, claw_current)]

        # Move to the bin and release the object
        actions.append(('translate_x', translations[0]))
        actions.append(('translate_y', translations[1]))
        actions.append(('translate_z', translations[2]))
        actions.append(('release',))

        # Update claw position and power used
        claw_current = nearest_bin
        power_used += sum(abs(t) for t in translations)

        # Remove the placed object and bin from the lists
        objects_initial.remove(nearest_object)
        bins.remove(nearest_bin)

    if objects_initial:
        return "No solution found within power limit"
    else:
        return actions

    \end{gptcodeblock}
\end{gptresponse}
\end{chat}
\caption{\label{fig:claw1} \gpt provides a greedy approach to the problem of minimizing the distance traveled by the claw, which does not guarantee an optimal solution. }
\end{figure}

Though GPT understands that it needs to keep track of the position of the claw to compute the correct distances and that the claw should move to an object before moving to a bin, it does not able to output an optimal solution, even when the problem statement limits the total number of objects and bins. We thus directly specify while prompting that the outputted function should guarantee that the minimum distance is traveled. 

\begin{figure}[h]
\begin{chat}{false} % param: prevent page breaks in chat (true=page breaks allowed, false=not allowed)

\begin{userprompt}{0.0\textwidth}{} 
Could you write a function that guarantees the global optimum? Make sure to account for the distances from the claw to object and claw to bin (after it has grasped the object). Also make sure to compute translations rather than Euclidean distance. Recall the bounds are 0 <= n <=3 and 0 <= m <= 3.
\end{userprompt}

\begin{gptresponse}{0.0\textwidth}{} 
...text omitted for brevity...\
   
This updated function generates all permutations of the objects and bins, calculates the total translation required for each permutation, and selects the one with the smallest total translation. 

\begin{gptcodeblock}{Python}
from itertools import permutations

def move_arm(claw_initial, objects_initial, bins, T_max):
    def translation_distance(p1, p2):
        # Calculate Manhattan distance (total translation) between two points
        return abs(p1[0] - p2[0]) + abs(p1[1] - p2[1]) + abs(p1[2] - p2[2])
    
    def calculate_total_translation(ordering):
        total_translation = 0
        claw_pos = list(claw_initial)
        
        for object_pos, bin_pos in ordering:
            total_translation += translation_distance(claw_pos, object_pos)  # Claw to object
            total_translation += translation_distance(object_pos, bin_pos)  # Object to bin
            claw_pos = bin_pos  # Claw is now at bin location
            
        return total_translation
    
    object_bin_pairs = list(permutations(zip(objects_initial, bins)))
    
    min_translation = float('inf')
    best_ordering = None
    
    for ordering in object_bin_pairs:
        total_translation = calculate_total_translation(ordering)
        
        if total_translation < min_translation:
            min_translation = total_translation
            best_ordering = ordering
            
    if min_translation > T_max:
        return "No solution found within power limit"
    else:
        actions = []
        claw_current = list(claw_initial)
        for object_pos, bin_pos in best_ordering:
            # Move to object
            actions.extend([
                ('translate_x', object_pos[0] - claw_current[0]),
                ('translate_y', object_pos[1] - claw_current[1]),
                ('translate_z', object_pos[2] - claw_current[2]),
                ('grasp',)
            ])
            claw_current = list(object_pos)
            
            # Move to bin
            actions.extend([
                ('translate_x', bin_pos[0] - claw_current[0]),
                ('translate_y', bin_pos[1] - claw_current[1]),
                ('translate_z', bin_pos[2] - claw_current[2]),
                ('release',)
            ])
            claw_current = list(bin_pos)
        
        return actions
    \end{gptcodeblock}
\end{gptresponse}
\end{chat}
\caption{\label{fig:claw2} Though \gpt attempts to solve the minimum translation problem in a brute force manner, it fails to check all possible paths that the claw can take. }
\end{figure}

As seen in Fig. \ref{fig:claw2}, the code does not consider all possible bins that an object can be placed in once it has been picked up. We note that the solutions have high variance -- on a different run, \gpt does produce a correct brute force solution. A third rerun produces code that guarantees an optimal solution but is less efficient as it computes the translation for paths that do not obey the constraint that a claw must pick up an object before placing it in a bin.

% GPT (Version 2):
% \begin{lstlisting}
% Given the constraints you've provided and since the problem is constrained to small numbers of objects and bins (each less than or equal to 3), it's feasible to use a brute-force method to find the optimal solution. We will generate all permutations of objects and bins, compute the total energy cost for each permutation, and return the one with the minimum energy cost.

% Here is the function:

% ```python
% import itertools
% import math

% def optimal_arm_movement(claw_initial, objects_initial, bins, T_max):
%     def translation_distance(p1, p2):
%         # Calculate total translation distance between two points
%         return abs(p1[0] - p2[0]) + abs(p1[1] - p2[1]) + abs(p1[2] - p2[2])

%     best_actions = None
%     min_energy = float('inf')

%     # Generate all permutations of objects and bins
%     object_orders = list(itertools.permutations(objects_initial))
%     bin_orders = list(itertools.permutations(bins))

%     for object_order in object_orders:
%         for bin_order in bin_orders:
%             actions = []
%             energy = 0
%             claw_pos = claw_initial

%             for obj, bin in zip(object_order, bin_order):
%                 # Move to object
%                 actions.append(('translate_x', obj[0] - claw_pos[0]))
%                 actions.append(('translate_y', obj[1] - claw_pos[1]))
%                 actions.append(('translate_z', obj[2] - claw_pos[2]))
%                 actions.append(('grasp',))
%                 energy += translation_distance(claw_pos, obj)
%                 claw_pos = obj

%                 # Move to bin
%                 actions.append(('translate_x', bin[0] - claw_pos[0]))
%                 actions.append(('translate_y', bin[1] - claw_pos[1]))
%                 actions.append(('translate_z', bin[2] - claw_pos[2]))
%                 actions.append(('release',))
%                 energy += translation_distance(claw_pos, bin)
%                 claw_pos = bin

%                 if energy > T_max:
%                     break

%             # Update best actions if this order uses less energy
%             if energy < min_energy:
%                 best_actions = actions
%                 min_energy = energy

%     if best_actions is None:
%         return "No solution found within power limit"
%     else:
%         return best_actions

% claw_initial = (0, 0, 0)
% objects_initial = [(10, 10, 0), (20, 20, 0), (30, 30, 0)]
% bins = [(5, 5, 0), (15, 15, 0), (25, 25, 0)]
% T_max = 200

% print(optimal_arm_movement(claw_initial, objects_initial, bins, T_max))
% ```

% This function works by generating all permutations of objects and bins, then for each permutation, it calculates the total energy required to move the claw to each object, grasp it, move to the corresponding bin, and release the object. The permutation with the minimum energy usage that does not exceed `T_max` is then returned. If no solution is found within the power limit, it returns a message indicating this. 

% Remember that this method, while it guarantees an optimal solution, could be computationally expensive and may not scale well for larger numbers of objects and bins. For scenarios with larger numbers of objects and bins, you might want to consider different algorithms like Greedy Algorithm, Genetic Algorithm, or other optimization techniques.

% \end{lstlisting}


% GPT (Version 3):
% \begin{lstlisting}
% Sure, with the constraint that we have 0 <= n, m <= 3, a brute force approach to solve this problem to find the globally optimal solution is feasible, considering every possible sequence of objects and bins.

% Here's how the function would look:

% ```python
% import itertools
% import sys

% def total_translation(path):
%     total = 0
%     for i in range(len(path) - 1):
%         total += abs(path[i][0] - path[i+1][0]) + abs(path[i][1] - path[i+1][1]) + abs(path[i][2] - path[i+1][2])
%     return total

% def find_optimal_path(claw_initial, objects_initial, bins, T_max):
%     # combine objects and bins in one list and permute them
%     objects_bins = objects_initial + bins
%     permutations = list(itertools.permutations(objects_bins, len(objects_bins)))

%     # add claw initial position as the start of each permutation
%     paths = [[claw_initial] + list(perm) for perm in permutations]

%     min_translation = sys.maxsize
%     optimal_path = None

%     for path in paths:
%         # check if the sequence of object and bin is valid (object followed by bin)
%         is_valid = True
%         for i in range(0, len(path) - 1, 2):
%             if path[i] in objects_initial and path[i+1] in bins:
%                 continue
%             else:
%                 is_valid = False
%                 break
        
%         if not is_valid:
%             continue

%         translation = total_translation(path)

%         if translation < min_translation and translation <= T_max:
%             min_translation = translation
%             optimal_path = path[1:]

%     if optimal_path is None:
%         return "No solution found within power limit"
    
%     return optimal_path

% claw_initial = (0, 0, 0)
% objects_initial = [(10, 10, 0), (20, 20, 0), (30, 30, 0)]
% bins = [(5, 5, 0), (15, 15, 0), (25, 25, 0)]
% T_max = 200

% print(find_optimal_path(claw_initial, objects_initial, bins, T_max))
% ```

% In the above function, the `find_optimal_path` function generates all permutations of objects and bins, checks if each permutation is a valid sequence (object followed by bin), and then finds the one with the minimum total translation that does not exceed the maximum allowed. If no valid path is found within the power limit, it returns a message indicating this.
% \end{lstlisting}

% Version 3 combines the object and bin positions into a single list and checks if permutations of the combined list are valid. However, this is a less efficient implementation as many permutations will be invalid solutions.
TODO: \url{https://chat.openai.com/share/828d9af0-2c88-4a0e-92da-9c33aec2dc67} --- analytical optimization and its limitations.

%A fundamental aspect of design involves searching for solutions that achieve optimal performance. This can be computationally intensive, particularly if the domain is expansive and if performance evaluation is computationally demanding. Typical approaches first establish a bounded design space to be searched over, and define objectives that can be computationally evaluated. We have already discussed both these factors in previous sections. The next step is to select the best algorithm to explore this domain, while taking into account various considerations - Is the domain discrete or continuous? Can we compute derivatives? How expensive is it to evaluate the objectives? How many objectives do we have and, if more than one, are they conflicting?

%Considering this landscape, one way GPT can support designers is by aiding them in finding the most effective method to execute the search when the domain and objectives are well-defined. We can also contemplate how GPT might handle multi-objective optimization, guiding users through a potentially complex landscape of trade-offs.

%Moreover, the creation of the design space can present challenges, as designers must clearly define boundaries, a task that can be difficult. In addition, some objectives may be challenging to quantify, as discussed in the previous section. In this context, we could consider whether GPT can propose novel strategies that free  designers from some of the typical burdens associated with the optimization pipeline.




%NOTES:
% Case 1: How good is it in search when it is given a design space and a metric?
% 1.1 can it just find the solution 
% 1.2 can it generate a correct algorithm that finds the solution?
% conclusion: maybe but is really that much better than not using it?
% examples: Robot arm -> shows that 1.2 does work (done) simple test: see if robot arm works for 1.1 
% Question: what other performance metrics we can (see if we can use stuff from the performance team)



Interesting design problems:
Look at the cartesian product of:

Analytical vs. simulation in the loop.

Constraints: Continuous, discrete, equality, bounded
Performance metrics: Continuous, discrete, binary, real-world only
Design space: Continuous, discrete, structured (graph?), unbounded vs. bounded
Multi-objective?

Examples: Format is Constraint type, Performance Metric, Design Space type

Robot arm: Continuous equality, continuous, Continuous bounded
Quadcopter: Continuous equality, continuous and real-world, Continuous bounded
Furniture (stabilization): None or material use (continuous), Binary (does it stand?), Unbounded
Will also come up with some purely analytical examples for these, or try solving some of these in an analytical way.

Can we do a simple stochastic turbulent flow example?


\paragraph{\textbf{Q2} Can GPT assist designers in navigating the landscape of possible trade-offs when multiple conflicting objectives are present?}

\paragraph{\textbf{Q3} Can GPT support design exploration and optimization when the design space is not properly defined or fully bounded?}

% NOTES:
% Case 2: what happens when the design space is ill-defined? 
% - can it maybe stay within some reasonable bounds which would be hard to do without some kind of domain understanding
%come up with an example where something is unbounded and see if chatgpt can optimize it? 
%system identification?

\paragraph{\textbf{Q4} Can GPT support design optimization when objectives are not easily quantifiable?}
Case 3: what happens when the performance metrics are more abstract?
again here we should talk to perfomance team! 















































% Inverse Design: What are the questions that we're trying to answer?

% 0. What is inverse design?

% 1. What is GPT capable of?

% 2. Where does it struggle?

% 3. Where does it need help?  i.e. what human problem-solving priors need to be placed on the workflow of generating solutions.

% 4. What external tools does GPT need to leverage or what custom tools do we need to develop as glue and tell GPT that they exist.


% -In this section, we:

% a) Provide a description of the inputs and ouptputs of inverse design.

% b) Provide a working example (TBD) showing how all aspects of design optimization can be generated using GPT.

% c) Show a ``Zoo'' 

%\paragraph{Overview}



\iffalse


\paragraph{Overview}
If you just specify, I want a table that can support 100kg, this might not work. You need to specify what the design space is. You need to specify some design space for tables.
Let's give a simple example of this.

The output is a design (specified as some point in the design space). One specific table that can do the job. It might be also possible that none of these design can satisfy the goals. 

\paragraph{Specifying Performance Goal}
This can be minimum (e.g., design with minimum performance in the set), maximum, given value (supports at least 100kg).

In the case of generative design, the output could be a collection of different designs.  One may desire to optimize over statistics of that set, \textit{e.g.}: maximize diversity (standard deviation) and so on.


\paragraph{Constraints on Performance Goal}
In either case, constraints may come into play.  "I only have 10 kg of material to work with" or "Ensure that the robot uses no more than its battery life to complete its task."  This can be especially challenging in the case of collection outputs, as different objectives, such as optimization, diversity, and parsimony can be in direct conflict with one another.

\paragraph{Examples}
"Make me a table that supports a person with as little compliance as possible with the amount of material I have on hand."

"Make me four robots with as different shapes as possible according to Hausdorff metric that complete a task in 1 minute."

design iteration based on what we think will work (using LLM or other tools), resampling from design space.

\fi
\fi

\subsection{Discussion}
TODO: format and expand.


The good:
1. Able to find an adequate choice for an algorithm for many problems - Able to also justify it - it doesn't always give you options right out of the gate - can sometimes get confused and rely on the domain to choose the algorithm.
2. Autocompletes a lot of content even before you ask (parameter bounds, constraints, objective function)
3. Can transfer some knowleldge to novel domains based on components - it can be fooled.
4. When the problem has an intuitive answer, can sometimes give that directly. (but can a user trust that?)

The Bad:
1. Some domains, ChatGPT will assume that it knows libraries that don't exist.  This also came up in performance evaluation.
2. Sometimes runs into memory issues setting up the problem.
3. Bad at spaital reasoning.

The Ugly:
1. Plugins can help, but sometimes lead to trouble.
2. Not always choosing the absolute best algorithm, especially if code doesn't exist.  So don't expect the most advanced algorithm.
3. Doesn't always set up problems in the most efficient way (e.g. analytical gradients)

==> sections/GraphArrows/TextToDesignExperiments/CAD_Fusion_basicDesigns.tex <==
%% Text to Design: CAD with Fusion360
% \team{Pingchuan, maybe with input from Mike}

if possible, example; though you mentioned the API changed too dramatically after end of GPT training window in Sept 2021 -- perhaps we could include this as a limitation?

==> sections/GraphArrows/TextToDesignExperiments/CAD_OnShape_multiPartAssemblies.tex <==
%% Text to Design: CAD with mating assemblies
% \team{Felix}

CSG and parametric CAD modeling paradigms are mainly used to design 3D parts which can be later on manufactured.
Putting these parts together into one functional object is usually done in an \textit{assembly} step.
In an assembly, specifying how two parts are connected, or \textit{mated}, comes down to defining (i) \emph{where} two parts are mated and (ii) \emph{what} the movement constraints are between two parts.
For example, to mate two lego bricks, we would define (i) the mate connector of the first brick on the top disk of one of its knobs, the mate connector of the second brick on the inner disk of its bottom tube and (ii) define the mate type as a sliding mate, allowing for a vertical translational degree of freedom (DOF). \todo{Lego mating figure}

In commercial CAD software, assemblies are defined via graphical interactions, allowing users to easily reason spatially and to correct their mate definitions thanks to real-time feedback.
GPT and other {\llm}s are purely text based, so they seem like a suboptimal choice for assembly. 
However, prior research has shown that \gpt has a good understanding over contextual and part relationships \cite{}, which could be useful for facilitating the mating process.

As for the parametric CAD modeling paradigms, we try to overcome the domain gap between the textual and the graphical domain by providing \gpt with a simplified DSL to express a minimal set of mating operations.
We define two operators: (i) an operator \lstinline{choose_planar_face(solid_name, plane_side)} which returns a mate connector based on the selected solid and its planar face and (ii) three mating operators \lstinline{mate}, \lstinline{mate_slider} and \lstinline{mate_revolute} which take as input two mate connectors and mate with either no DOF, one translational DOF and one rotational DOF, respectively.
\lstinline{mate_slider} and \lstinline{mate_revolute} additionally take the translation axis and the revolution axis as input argument.

For example, the program in Fig.\ref{fig:mate_stack_cuboids} (a) shows how to stack two cuboids on top of each other with this language.
Given our DSL definition, and this example program, \gpt can successfully stack three cuboids on top of each other, as is shown in Fig.\ref{fig:mate_stack_cuboids}(b) and (c). 
This simple example shows an important strength of \gpt, namely that it can learn from examples and is able to translate this to similar problems.
When assembling an object with a lot of parts and connectors, time-intensive manual labor is required to perform repeating patterns of mating operations \cite{automate}.
Leveraging {\llm}s which can reason about part relationships could prove to be a real time saver for designers.
\todo{}
In Fig.\ref{fig:mate_screws}, we see an example of a screw mating pattern which is performed once and which has to be repeated three more times in the remaining corners of the plate.
When asked to complete the assembly process, \gpt finishes the mating job successfully. 
It should be noted that the variables used in this example are explicitly descriptive.
\gpt performs less well when presented with no semantic context.
\\
\todo{}
\begin{itemize}
    \item explain slider mate example: place a drawer in a box
    \item failure case/limitation: 
    \item explain revolute mate example: door and hinge
    \item failure case/limitation:
\end{itemize}
Our mating DSL for \gpt shows potential benefits for real-world design scenarios, but also some limitations. 
It should be noted that the proposed DSL stays close to current graphical workflow.
Other DSLs could be better suited to interface with \gpt and maybe allow it to textually describe matings more naturally.
\\


==> sections/GraphArrows/TextToDesignExperiments/CSG_customPrimitives_integratingPrefabbedParts.tex <==
%% Text to Design: CSG with custom primitives, incorporating pre-fabbed parts 
% \team{Bohan}

wheels on Bohan's dresser/chest of drawers example.


==> sections/GraphArrows/TextToDesignExperiments/Electronics_Gerber_basicDesigns.tex <==
%% Text to Design: PCB specification from Gerber file
% \team{Young, maybe with input from Alyssa/Mike}


Designs with pre-defined schematics (imported components), use chatgpt to generate command for pcb layout variation.
electronics example of 8 LEDs as an array, 8:1 multiplexer, ADC, and microcontroller (arduino). Use KiCAD and python-based code

==> sections/capabilities.tex <==
\subsubsection{Observed Capabilities and Limitations} \label{sec:capabilities}

Our examination of \llm's performance in the fields of design and manufacturing has underscored several crucial capabilities instrumental in supporting the design processes, in addition to pinpointing significant limitations. \amy{underscored that \gpt has several crucial capabilities, or \gpt needs these capabilities? Or that we think these should be capabilities \gpt has that would be useful? It feels a little weird to have a discussion about our observations on what \gpt can do before we've shown the evidence we observed it from} Next, we outline these observations and discuss various methods to mitigate the identified limitations. Each of these points will be further detailed and exemplified in the following sections.

\noindent \textbf{Capabilities:} \linebreak
\noindent \textbf{C.1 Extensive Knowledge Base in Design and Manufacturing:} \llm boasts a comprehensive knowledge base in the realms of design and manufacturing. Its capabilities extend to solving a wide array of problems and automatically completing specifications, making it a versatile tool across various domains.

\noindent \textbf{C.2 Iteration Support:} \llm incorporates an iterative approach to problem-solving. When feedback is provided on errors, it attempts to rectify them. This ability to adapt and learn, \amy{might be worth clarifying what "learning" means here (incorporating past responses? collecting data?) since that is a term of art...} although not always successful, is a valuable facet of an \llm's performance.

\noindent \textbf{C.3 Modularity Support:} \llm supports modular design, demonstrating the ability to reuse or adapt previous designs or solutions when explicitly instructed. While it does not inherently retain memory of past interactions, explicit instructions can help leverage its modular capabilities effectively.


\noindent \textbf{Limitations:} \linebreak
\noindent \textbf{L.1 Reasoning Challenges:} \llm encounters difficulties with certain types of reasoning, particularly those involving analytical reasoning and computations. These limitations can manifest as notable challenges in the design and manufacturing domain, for instance, a general lack of spatial reasoning capabilities.

\noindent \textit{Potential Solutions:} Implementing well-crafted domain-specific languages (DSLs) can help address these challenges. DSLs, widely used in computer science, encapsulate recurring knowledge, rules, and valuable abstractions, thereby filling knowledge gaps. Alternatively, APIs that can perform the complex computations can be integrated. \llm's proficiency in creating high-level abstractions can be utilized to generate inputs that be processed through APIs by computational solvers.

\noindent \textbf{L.2 Correctness and Verification:} \llm often produces inaccurate results or justifications for its solutions and lacks the ability for self-verification.

\noindent \textit{Potential Solutions:} Apart from relying on human verification, automated verification can be accomplished by utilizing APIs that conduct checks and validations. By leveraging \llm's iterative capabilities (C.2), we can create a feedback loop that continues until a satisfactory solution is obtained.

\noindent \textbf{L.3 Scalability:} As tasks become larger or more complex, \llm's performance can deteriorate, often struggling to manage multiple tasks concurrently.

\noindent \textit{Potential Solutions:} One strategy is to partition larger tasks into multiple sub-tasks. For instance, rather than requesting it to evaluate multiple performance metrics simultaneously, it may be more effective to request them individually. When constructing more complex models, employing an incremental design process can prove beneficial. Components can be designed and verified separately before being assembled into the final model. \llm's modularity support (C.3) can be used to facilitate the creation of complex models from a series of instructions.

\noindent \textbf{L.4 Iterative Editing:} When a design needs modifications, specifying those changes as a prompt will often lead to unsatisfactory behaviors. This is because the \llm, upon receiving a change prompt, will regenerate the design, often overlooking elements specified in previous prompts. This situation poses challenges to design editing.

\noindent \textit{Potential Solutions:} Our solutions involved either feeding the prompts back in to create a full specification in a single prompt, though this also caused challenges due to the scalability limitations discussed above. The alternative was explicit modularization to enable parts to be designed and reused, though the latter was not possible in some cases.

\noindent \textbf{Dualism:}

\noindent \textbf{D.1 Context Information:} \llm's performance improves significantly with the provision of context information. The more detailed the domain description, the better it performs. Furthermore, \llm is adept at providing context for its actions, making it an asset in sequential workflows. This characteristic proves particularly beneficial when using \llm generated content in subsequent tasks, as these tasks can utilize the context included in the output from the initial task.
\noindent \textbf{D.2 Unprompted Responses:} \gpt often infers aspects that are not specified in the prompt, either auto-completing specifications or finding ways to make decisions without enough information. While this is interesting in the design context in terms of allowing for partial specifications that can be auto-completed, it can sometimes be overly proactive, guiding the design in some aspects, which may limit creativity.




==> sections/limitations.tex <==
\section{Limitations}

Describe limitation of each of the components of the workflow

\paragraph{Text-To-Design}
What are the limits on design primitives?
What are the limits of constraints?
What are the limits on modularity/hierarchical design?

Evaluate validity of the design.
Evaluate correctness.

\paragraph{Text-To-Design-Space}
Limits of parametric design.
Limits of interpolation/extrapolation.
Limits of grammars.

\paragraph{Design-To-Manufacturing}
Limits of validity of the translation.
Limits of correctness.
Limits on the length of the output. Complexity of the output.
Limits on custom manufacturing processes.

\paragraph{Design-To-Performance}
Which performance metrics are understandable?
Which performance metrics need external simulation?

\paragraph{Performance-and-Design-Space To Design}
Which objective function are understandable?
What are the limits on specifying constraints?
What are the limits of the search process for the inverse?



==> sections/result-copter-old.tex <==




\liane{this section feels a bit out of order at the moment -- by the end of 9.2.2 we have a fabbed frame; then 9.2.3 talks about sim without making any link back to how/whether the sim is used for the real world example; then 9.2.4 talks about selecting the components, around which the frame from earlier was designed. I think reordering this [e.g., sourcing --> generic frame design --> (sim?) --> manufacturing considerations --> real object] could make it a lot less confusing. }

\subsubsection{Text-to-Design}
\label{sec:copter-text-to-design}

We use \gpt to generate a javascript program using our custom defined box function and cylinder function, as described in Section~\ref{sec:prefabbed-ele}. The implementation of the box function is based on \jscad, so we can use the online \jscad viewer to directly export an STL file for later manufacturing. The details are explained in Section~\ref{sec:prefabbed-ele}.

\adriana{what about component selection here?}

\subsubsection{Design-to-Manufacturing}
\label{sec:copter-manufacturing}

\begin{figure}[H]
\includegraphics[width=\textwidth]{figures/quadcopter-man.png}
\caption{The quadcopter frame.}
\label{fig:quadcopter-man}
\end{figure}

Our approach is streamlined by using an STL file described in Section~\ref{sec:copter-text-to-design}. 
As mentioned earlier, the design uses several existing parts, and it is difficult to describe the geometric details of each part.
Moreover, \gpt does not understand how to make the frame such that the quadcopter is physically balanced.
Thus, we do not directly ask \gpt to create a manufacturable frame that all parts can be mounted onto, but instead we issue low-level instructions to guide \gpt to 
generate a valid frame.
%We follow the steps in Section~\ref{sec:additive} to convert our language-based design to an STL that can quantitatively describe the geometry of the designed copter's frame.
%\FH{what do you mean by quantitatively? Doesn't it just describe the geometry?}

We first adjust the size of the frame bar cross section through \gpt
so it is 3D printable and sufficiently stiff.
Then, we union all the boxes and cylinders that belong to the frame.
The battery is placed such that half of it is sunken into the frame, 
and then we subtract it from the frame.
This gives the final frame.
Next, we consider how the remaining parts will be mounted onto the frame.
The battery does not require any further modification to ensure a secure attachment, because the frame will hold the battery tightly by construction.
For the controller and the signal receiver,
they can be glued to the battery, so no additional handling is needed as well.
Finally, for the motors, they are mounted using screws.
so there should be screw holes on the frame.
We would like to use \gpt to make holes
and see how far it can proceed to solve this problem.
For each motor, we ask \gpt to generate 4 cylinders that represent the needed holes.
We use text to describe the specification of the holes to \gpt.
Although the mounting holes are not trivial,
we were still able to get the correct cylinders after a few iterations with \gpt.
They are shown in dark gray in Figure~\ref{fig:quadcopter-man}(Left).
Once the hole cylinders for one motor is ready,
we let \gpt group them and duplicate them using our \lstinline{place} function.
This again poses difficult mathematical problems to \gpt.
We were able to get the hole cylinders to be placed into the correct position, 
but we couldn't achieve the correct rotation.
This is later fixed by manually adjusting the angle.
As we can see, the hole cylinders are overlapping with the frame bar.
Because we cannot change the thickness of the frame bar, 
we have to adjust the thickness of the tip of the frame bar 
so that it does not block the holes.
This part is also achieved manually 
because we found it difficult to describe the problem and the solution to \gpt.

Another limitation we found during our experiments is that 
it is difficult to tweak the designs we finished earlier.
After a long conversation with \gpt, it becomes difficult to communicate with it
about the topics we have designed earlier.
As a result, if we find any issues in the part we addressed earlier,
it is hard to bring it up again to \gpt and let it make changes.
In other words, it would be ideal if one could finish any design without the need to re-touch it at any future point.
Otherwise, it would be challenging to re-adjust it later.
The final result of the frame is shown in Figure~\ref{fig:quadcopter-man}(Right).
Overall, with the aid of a user, we can design a manufacturable quadcopter through \gpt.  \adriana{good point we don't talk so much about iterations, probably worth bringing it to the broader discussion. }

\adriana{everything up until here sounded like design, I don't understand why it's in the fabrication section and how it realtes to the design section above.}

Once the frame is determined, we use a 3D printer to create the frame of the copter. The printer is a Fortus 400, a model renowned for its high-performance and precision manufacturing capabilities, making it ideally suited to the task at hand. Its substantial build volume, one of its standout features, is especially advantageous for larger projects like the copter. This is crucial given the sizeable dimensions of the copter, which could potentially outsize the build volume of many other printer models.

The Fortus 400 is capable of Fused Deposition Modeling (FDM) technology, a popular form of additive manufacturing where layers of heated and extruded thermoplastic are successively laid down according to the design's geometry. This makes it an excellent choice for creating robust, durable parts like the quadcopter frame we intend to manufacture.
\FH{The way you describe the 3D printer makes it sound like you are paid by Fortus. I don't think you have to justify why you chose a particular 3D printer, just say we print it.}
\liane{seconded; I'd probably summarize these two paragraphs by saying "Once the frame is determined, we fabricate it using a 3D printer. We use the Fortus 400, because it has a sufficiently large build volume and it realizes precise, robust, and durable parts.}

We instruct the printer to use the least amount of infill possible in the print settings. By choosing a lower infill percentage, the printer will create a sparse or hollow internal structure rather than a solid one. This decision helps conserve material and reduce print time without significantly compromising the strength or weight of the copter's frame, given that it is not a load-bearing component.

% By leveraging the advanced capabilities of the Fortus 400 3D printer and the efficiency of the infill pattern, we are able to produce a high-quality copter frame that
The resulting fabricated copter frame
not only meets the required dimensions, but also balances the strength and weight, necessary for optimum flight performance. We visualize the printed frame in Figure~\ref{fig:copter-frame}.

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{figures/frame.jpg}
    \caption{\label{fig:copter-frame}}
\end{figure}


\subsubsection{Text-to-Performance}

% Leader: Megan, Edward, Andy

We use \gpt to measure the quadcopter's performance through simulation. As described in Section~\ref{sec:quadcopter_sim}, this first involves converting a given \jscad design to a format amenable to simulating multibody robots, such as URDF. We then prompt \gpt to provide a LQR controller which takes in both the design in URDF format and relevant physical properties. We also describe in Section~\ref{sec:quadcopter_sim} how the quadcopter's design can be optimized through simulation. \liane{do you use these results for the fabricated example? right now feels a bit whiplash-y to go to from fab back to simulation with no tie-in for how/if the sim is applied to the real world example}


\subsubsection{Real-world example}
\liane{this header seems weird (in the cabinet section too). maybe fabricated example? [coordinate with cabinet folks to pick a consistent title]}

%We follow the operation from the previous sections and ask \gpt for the best out-of-shelf components we can get from the market.

The previous examples evaluate the text-to-design capabilities of \gpt in a CAD-like setting by constructing objects from basic primitives. However, many real-world systems such as drones are constructed from pre-designed components with varying specifications. This next example examines the ability of \gpt to select real-world components for a specific use case: constructing an indoor drone capable of a given speed.
\liane{I don't think you need to summarize/motivate here -- we've already done that in the paper. I'd just say "Now we want to create a real-world drone capable of achieving a given speed"}



\begin{chat}{false}

\begin{userprompt}{0\textwidth}{}
Which components do I need to build an indoor drone that can fly at 30 mph? Prefer easily available components if possible. List the manufacturer, model, quantity, and Amazon search term for each component.

Next, write a Python function that constructs the drone. The following functions are available to use:

\begin{gptcodeblock}{Python}
add_cylindrical_component(manufacturer: str, model: str, mass_grams: float, diameter_mm: float, height_mm: float, parent: int) -> int: Adds an instance of a cylindrical component and returns its ID. The new instance is attached to the instance with ID `parent`.
add_cuboid_component(manufacturer: str, model: str, mass_grams: float, length: float, width_mm: float, height_mm: float, parent: int) -> int: Adds an instance of a cuboid component and returns its ID. The new instance is attached to the instance with ID `parent`.
\end{gptcodeblock}
\end{userprompt}

\begin{gptresponse}{0\textwidth}{}
Building an indoor drone that can fly at 30 mph requires several components. Here's a list of the necessary components along with their specifications and Amazon search terms:

\begin{enumerate}
    \item Frame:
    \begin{itemize}
        \item Manufacturer: Hobbypower
        \item Model: Hobbypower F450
        \item Quantity: 1
        \item Amazon search term: Hobbypower F450 frame kit
    \end{itemize}

    \item Flight Controller:
    \begin{itemize}
        \item Manufacturer: Holybro
        \item Model: Kakute F7 Mini
        \item Quantity: 1
        \item Amazon search term: Holybro Kakute F7 Mini flight controller
    \end{itemize}

    \item Motors:
    \begin{itemize}
        \item Manufacturer: EMAX
        \item Model: EMAX RS2205S
        \item Quantity: 4
        \item Amazon search term: EMAX RS2205S motors
    \end{itemize}

    \item Electronic Speed Controllers (ESCs):
    \begin{itemize}
        \item Manufacturer: Hobbypower
        \item Model: Hobbypower SimonK 30A
        \item Quantity: 4
        \item Amazon search term: Hobbypower SimonK 30A ESC
    \end{itemize}

    \item Propellers:
    \begin{itemize}
        \item Manufacturer: DALPROP
        \item Model: DALPROP T5045C
        \item Quantity: 4 pairs (8 propellers)
        \item Amazon search term: DALPROP T5045C propellers
    \end{itemize}

    \item Battery:
    \begin{itemize}
        \item Manufacturer: Tattu
        \item Model: Tattu 4S 1300mAh
        \item Quantity: 1
        \item Amazon search term: Tattu 4S 1300mAh LiPo battery
    \end{itemize}

    \item Radio Transmitter and Receiver:
    \begin{itemize}
        \item Manufacturer: FrSky
        \item Model: FrSky Taranis X9D Plus
        \item Quantity: 1
        \item Amazon search term: FrSky Taranis X9D Plus transmitter and receiver
    \end{itemize}

    \item Power Distribution Board (PDB):
    \begin{itemize}
        \item Manufacturer: Matek Systems
        \item Model: Matek PDB-XT60
        \item Quantity: 1
        \item Amazon search term: Matek PDB-XT60 power distribution board
    \end{itemize}

    \item Propeller Guards (optional but recommended for indoor use):
    \begin{itemize}
        \item Manufacturer: Crazepony
        \item Model: Crazepony 2 Sets 65mm
        \item Quantity: 1 set
        \item Amazon search term: Crazepony 65mm propeller guards
    \end{itemize}
\end{enumerate}

Now, let's write the Python function to construct the drone using the provided functions:

\begin{gptcodeblock}{Python}
def construct_indoor_drone():
    # Add frame
    frame_id = add_cuboid_component("Hobbypower", "Hobbypower F450", 300, 450, 55, 55, 0)
    
    # Add flight controller
    fc_id = add_cuboid_component("Holybro", "Kakute F7 Mini", 15, 35, 35, 10, frame_id)
    
    # Add motors
    motor_ids = []
    for _ in range(4):
        motor_ids.append(add_cylindrical_component("EMAX", "EMAX RS2205S", 30, 28, 17.5, frame_id))
    
    # Add ESCs
    esc_ids = []
    for _ in range(4):
        esc_ids.append(add_cylindrical_component("Hobbypower", "Hobbypower SimonK 30A", 15, 22, 6, frame_id))
    
    # Add propellers
    propeller_ids = []
    for _ in range(4):
        propeller_ids.append(add_cylindrical_component("DALPROP", "DALPROP T5045C", 5,
\end{gptcodeblock}
\end{gptresponse}

\begin{userprompt}{0\textwidth}{}
I already have a radio transmitter, please suggest a receiver only
\end{userprompt}

\begin{gptresponse}{0\textwidth}{}
Certainly! If you already have a radio transmitter and only need a receiver, you can consider the following option:

\begin{enumerate}
    \item Receiver:
    \begin{itemize}
        \item Manufacturer: FrSky
        \item Model: FrSky XSR
        \item Quantity: 1
        \item Amazon search term: FrSky XSR receiver
    \end{itemize}
\end{enumerate}

Please note that the FrSky XSR receiver is compatible with the FrSky Taranis X9D Plus transmitter, which you mentioned having.
\end{gptresponse}

\end{chat}
\FH{Please fix the page-break problems with this chat. You can break it up into multiple smaller chats and also only show relevant information.}
\liane{isn't a more space-efficient version of this exact conversation already included in the earlier sections? \fref{fig:copter-parts}. Could you just reference that?}
\liane{I see there's they python block which isn't in the original; if you really want this block, you can just use the omitted command to comment out the part list/reference the other fig and then include the python.}


The most common failure cases include suggesting nonexistent components, placeholder components (e.g. ``XYZ Motor''), and unnecessary components (e.g. ESCs \liane{I didn't know what an ESC was -- maybe define it once in the main text too, not just in the chat snippet} and power distribution board for an all-in-one controller). We found that requesting search terms for a specific online retailer \liane{such as?} resulted in fewer instances of placeholder components. The chosen components are generally electrically compatible, with the ESCs supporting the series cell count of the battery (e.g. 2S, 3S, 4S). Mechanical incompatibility is more of an issue, with propellers and motors occasionally having different shaft sizes. This is generally not an issue, however, since propeller manufacturers tend to include adapter rings with their products.\liane{nitpick, but weird phrasing with "mechanical incompatibility is more of an issue, ... This is generally not an issue"}

One significant strength of \gpt in this text-to-design scenario is that it can tailor the component selection to the use case. For example, specifying a ten-kilogram payload requirement will result in \gpt suggesting much larger motors and propellers. As demonstrated in the transcript \liane{which transcript?}, further interactions with \gpt can be useful for finding alternate components.

After verifying that the components are indeed compatible, we purchased them from an online retailer. Note that we omit the propeller guards and frame (which we manufacture using 3D printing) as well as the ESCs and power distribution board, which are included in the controller. We show the purchased components in Figure~\ref{fig:purchased}.

\begin{figure}[ht]
\centering
\includegraphics[width=\textwidth]{figures/purchased.jpg}
\caption{\label{fig:purchased} \FH{missing caption}}
\end{figure}




\liane{I would split the section here. Take all the \gpt-assisted part sourcing info and start the section with that; then talk about the frame design  + (maybe sim if relevant?) + frame manufacturing; then talk about assembly + testing }

After the 3D printed frame is prepared following Section~\ref{sec:copter-manufacturing}, the next step is the assembly of the copter with the mechanical components that have been prepared before. These components form the backbone of the copter's functionality and are crucial to its flight performance.

\FH{Do we need the explanation of the assembly? What is our message here? Does this have to do anything with the \gpt exploration?}\liane{I think it makes sense if focused on the interface between the \gpt-designed frame and the pre-fabbed parts. Not sure if we need the explanation of what each part does, but it does help justify the attachment mechanism some. The description is nice and I learned a lot from it, though -- I'd probably at least keep in an appendix if it gets nixed from the main text}
First, we have the flight controller, which serves as the brain of the copter. It integrates all sensor data, interprets inputs from the radio receiver, and makes necessary adjustments to the motors' power for maintaining stability and control during flight. This component is secured onto the copter frame using double-sided tape and wrappers to ensure a firm and secure fit, preventing it from moving or detaching during operation.

Next, we have 4 motors, which provide the power needed for the copter's propulsion and maneuverability. They are attached at each corner of the copter frame, maintaining an equidistant configuration for balanced performance. Attachment is done using screws, which provide a sturdy and reliable fastening method, ensuring that the motors stay firmly in place even under the high-speed rotation and vibrational forces experienced during flight.

Each motor is paired with a propeller, which converts the motor's rotary motion into lift, enabling the copter to ascend and descend. These are also affixed using screws, ensuring a secure fit to handle the high rotational speeds without risk of detachment or imbalance.

The battery, which provides the energy needed for the flight controller, motors, and other electrical components, is also fastened onto the frame using double-sided tape and wrappers. This positioning method allows for secure placement while also enabling easy access for battery replacement or recharging.

Finally, we have the radio receiver, which receives input signals from the remote control transmitter. It communicates these commands to the flight controller, initiating changes in flight direction, speed, and altitude. Like the flight controller and the battery, the radio receiver is attached to the frame using double-sided tape and wrappers, ensuring that it remains secure and stable during flight while still being easily accessible for maintenance or troubleshooting.

Each component plays a pivotal role in the operation of the copter, and the assembly process involves meticulous placement and secure attachment of each part. All elements are firmly and stably attached as shown in Figure~\ref{fig:copter-assemble}, creating a sturdy and reliable copter ready for flight.

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{figures/assemble.png}
    \caption{\label{fig:copter-assemble}}
\end{figure}

The final phase is a crucial real-world evaluation of the newly-assembled copter. This hands-on, operational testing allows us to assess and validate the functionality and performance of our copter under real-world conditions, ensuring it performs as intended.

First, we conduct an ascending test. This involves commanding the copter to lift off the ground and rise to a predetermined altitude. This test serves to evaluate the collective thrust of the motors and the performance of the propellers in translating the motors' rotary motion into lift. It also gives us a chance to observe the responsiveness of the copter to commands from the radio transmitter, the efficacy of the flight controller in interpreting these commands, and the general stability of the copter during ascent. We show the motion in Figure~\ref{fig:copter-flight-test} (left).

Following the ascent, the next stage of evaluation involves a hovering test. In this phase, the copter is commanded to maintain its altitude and position for a set duration. Hovering requires the continuous, simultaneous operation of all four motors to counteract the pull of gravity. This test is particularly revealing of the copter's ability to achieve and sustain stable flight, a critical attribute of any functional copter. We show the motion in Figure~\ref{fig:copter-flight-test} (mid).

Lastly, we conduct a descending test, commanding the copter to safely and smoothly lower itself back to the ground. This tests the copter's controlled reduction of thrust and the resultant downward movement, as well as the flight controller's ability to interpret and execute the descent command. It is also a critical test of the copter's landing capabilities, as a safe and smooth landing is vital to preserving the integrity of the copter and its components. We show the motion in Figure~\ref{fig:copter-flight-test} (right).

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{figures/placeholder.png}
    \caption{\label{fig:copter-flight-test}}
\end{figure}

